TypedMatrices.jl: An Extensible and Type-Based Matrix Collection for Julia

TypedMatrices.jl is a Julia package to organize test matrices. By default, the package comes with a number of built-in matrices and interfaces to help users select test cases based on their properties. The package is designed to be extensible, allowing users to define their own matrix types. We discuss the design and implementation of the package and demonstrate its usage with a number of examples.

==> features.tex <==
\section{Features and interfaces}



















































